Robust State Estimation from Partial Out-Core Measurements with Shallow Recurrent Decoder for Nuclear Reactors

Reliable, real-time state estimation in nuclear reactors is of critical importance for monitoring, control and safety. It further empowers the development of digital twins that are sufficiently accurate for real-world deployment. As nuclear engineering systems are typically characterised by extreme environments, their in-core sensing is a challenging task, even more so in Generation-IV reactor concepts, which feature molten salt or liquid metals as thermal carriers. The emergence of data-driven methods allows for new techniques for accurate and robust estimation of the full state space vector characterising the reactor (mainly composed by neutron fluxes and the thermal-hydraulics fields). These techniques can combine different sources of information, including computational proxy models and local noisy measurements on the system, in order to robustly estimate the state. This work leverages the Shallow Recurrent Decoder (SHRED) architecture to estimate the entire state vector of a reactor from three, out-of-core time-series neutron flux measurements alone. Specifically, the Molten Salt Fast Reactor, in the EVOL geometry (Evaluation and Viability of Liquid Fuel Fast Reactor System project), is demonstrated as a test case, with neutron flux measurements alone allowing for reconstruction of the 20 coupled field variables of the dynamics. This approach can further quantify the uncertainty associated with the state estimation due to its considerably low training cost on compressed data. The accurate reconstruction of every characteristic field in real-time makes this approach suitable for monitoring and control purposes in the framework of a reactor digital twin.

==> shred_theo.tex <==
\section{SHRED Theory}

The SHRED architecture is based upon the separation of variables technique for solving linear partial differential equations (PDEs)~\cite{folland2020introduction}.  Separation of variables assumes that a solution can be separated into a product of spatial and temporal functions $u(x,t)= T(t) X(x)$.  This solution form is then used to reduce the PDE into a ordineary differetial equations:  one for time $T(t)$ and one for space $X(x)$.  Such a decomposition also constitutes the underpinnings of spectral methods for the numerical solution of the PDE, linear or nonlinear~\cite{kutz:2013}.  

Consider the constant coefficient linear PDE 
%
\begin{equation}
 \dot{u} = {\cal L} (\partial_x, \partial^2_x, \cdots ) {u}
 {\label{eq:linearPDE}}
\end{equation}
%
where $u(x,t)$ specifies the spatio-temporal field of interest. Typically the initial condition (IC) and boundary conditions (BCs) are given by
%
\begin{subequations}
\begin{align}
\text{IC:}&&\quad  u(x,0)=u_0(x) \\
\text{BCs:}&&\quad  \alpha_1 u (0,t) +\beta_1 u_x(0,t) = g_1(t) \,\, \text{and} \nonumber \\  && \alpha_2 u(L,t) + \beta_2 u_x(L,t) = g_2(t).
\end{align}
\label{eq:ICBC}
\end{subequations}
%
This may be generalized to systems of several spatial variables, or a system with no time dependence.  The linear operator ${\cal L}$ specifies the spatial derivatives, which in turn model the underlying physics of the system.  Simple examples of ${\cal L}$ include ${\cal L}= c \partial_x$ (the one-way wave equation) and ${\cal L}= \kappa \partial^2_x$ (the heat equation)~\cite{kutz:2013}.  

The earliest solutions of linear PDEs assumed separation of variables whereby $u(x,t)=\exp(\lambda t) X(x)$ was a product of a temporal (exponential) function multiplied by a spatial function.  The parameter $\lambda$ is in general complex.  This gives the eigenfunction solution of (\ref{eq:linearPDE}) to be
%
\begin{equation}
    u(x,t) = \sum_{n=1}^{N} a_n \exp(\lambda_n t) \phi_n(x)
    \label{eq:ef}
\end{equation}
%
where $\phi_n(x)$ are the eigenfunctions of the linear operator and $\lambda_n$ are its eigenvalues (${\cal L}\phi_n(x) = \lambda_n \phi_n(x)$).  Here a finite dimensional approximation $N$ is assumed, which is standard in practice for numerical evaluation.  

Typically, initial conditions $u(x,0)=u_0(x)$ are imposed in order to uniquely determine the coefficients $a_n$.  Specifically, at time $t=0$ (\ref{eq:ef}) becomes
%
\begin{equation}
    u_0(x) = \sum_{n=1}^{N} a_n  \phi_n(x) .
\end{equation}
%
Taking the inner product of both sides with respect to $\phi_m(x)$ and making use of orthogonality gives
%
\begin{equation}
   a_n =\langle u_0(x), \phi_n(x) \rangle
\end{equation}
%
Instead of having the full spatial distribution at $t=0$ ($u_0$), SHRED has the measurements at a single spatial (sensor) location $x_s$, but with a temporal history.  Thus if SHRED has, for example, $N$ temporal trajectory points, this gives at each time point of the measurement:
%
\begin{equation}
    u(x_s, t_j) = \sum_{n=1}^{N} a_n 
    \exp(\lambda_n t_j) \phi_n(x_s) 
    \,\,\,\,\,\, \mbox{for} \,\,\, j=1,2,\cdots N .
\end{equation}
%
This results in $N$ equations for the $N$ unknowns $a_n$. Specifically, the $N\times N$ system of equations ${\bf A} {\bf x} = {\bf b}$ is prescribed by the vector components $x_k=a_k$ and $b_k = u(x_s,t_k)$ and matrix components $(a_{kj}) = \exp(\lambda_k t_j) \phi_k(x_s)$.  As with the initial condition (\ref{eq:ICBC}a), the time trajectory of measurements at a single location uniquely prescribes the solution.  This analysis can easily be generalized to include multiple sensor measurements at a single time point. Thus if there are two measurements at a given time $t_j$, then only $N/2$ trajectory points are needed to uniquely determine the solution.  Likewise, three sensor measurements at a given time requires on $N/3$ trajectory points.
%
In addition to stationary sensors measurements, one can also consider mobile sensors whereby the measurement of the system is a different locations over time:  $x_s = x_{s(t_j)}$. The above arguments are easily modified so that the vector component $b_k = u(x_{s(t_j)},t_k)$ and matrix components $(a_{kj}) = \exp(\lambda_k t_j) \phi_k(x_{s(t_j)})$.

Thus, temporal trajectory information at a single spatial location, or with a moving sensor, is equivalent to knowing the full spatial field at a given point in time. SHRED is a generalization of the separation of variables architecture $u(x,t) = T(t)X(x)$ where the LSTM models time $T(t)$ and the decoder models space $X(x)$.  Of course, as a generalization to nonlinear dynamics, rigorous theoretical bounds of SHRED are difficult to achieve, much like analytic and numerical solutions are difficult to rigorously bound in computational PDE settings.  But certainly in the linear limit, the above arguments show explicitly why SHRED is guaranteed to work and recover the full spatio-temporal field exactly.

\subsection{Nonlinear PDEs}

The above arguments show that time and space measurements can be traded for each other explicitly for linear PDEs.  For nonlinear PDEs
%
\begin{equation}
 \dot{u} = N (u, u_x, u_{xx}, \cdots ), 
 {\label{eq:nonlinearPDE}}
\end{equation}
%
numerical solution techniques are typically used to generate solutions subject to the initial and boundary conditions~(\ref{eq:ICBC}).  Consider a spectral solution technique~\cite{kutz:2013} whereby numerical solutions are approximated by a spectral basis
%
\begin{equation}
    u(x,t) = \sum_{n=1}^{N} a_n (t) \phi_n(x) .
    \label{eq:spectral}
\end{equation}
%
Typical examples of spectral techniques include using Fourier modes or Chebychev polynomial for $\phi_n(x)$.  This spectral decomposition turns the PDE into a systems of $N$ coupled ordinary differential equations for $a_n(t)$:
%
\begin{equation}
  \frac{da_n}{dt}=f_n (a_1, a_2, \cdots, a_N) \,\,\,\,\,\, \mbox{for} \,\,\, n=1, 2, \cdots N 
  \label{eq:an}
\end{equation}
%
The solution of the $N$-dimensional differential equation has $N$ unknown constants of integration that are typically uniquely determined by applying initial conditions and orthogonality in (\ref{eq:spectral})
%
\begin{equation}
    a_n(0)= \langle u_0(x), \phi_n(x) \rangle   . 
\end{equation}
%
As with the separation of variables solution, we can instead assume that we can construct a general solution  for
(\ref{eq:an}) which has $N$ constants of integration. The constants of integration can be determined by requiring the solution to satisfy $N$ temporal trajectory points, giving at each time point of the measurement:
%
\begin{equation}
    u(x_s,t_j)=\sum_{n=1}^N a_n(t_j)\phi_n(x_s)  \,\,\,\,\,\, \mbox{for} \,\,\, j=1,2,\cdots N .
\end{equation}
%
This gives $N$ constraints for the $N$ unknown constants of integration, thus uniquely determining the evolution of the $a_n$ in (\ref{eq:an}).  Mobile sensors can also be used to enforce the constraints required for a unique solution.\\


\subsection{Coupled PDEs}

We can also consider coupled, constant coefficient linear PDEs.  For example, the coupled system 
%
\begin{subeqnarray}
 \dot{u} = {\cal L}_1  {u}
 + {\cal L}_2  {v}\\
 \dot{v} = {\cal L}_3  {u}
 + {\cal L}_4 {v}
 {\label{eq:linearPDE2}}
\end{subeqnarray}
%
where $u(x,t)$ and $v(x,t)$ specifies the spatio-temporal fields of interest. The PDEs can be instead be written in the form
%
\begin{equation}
    \ddot{u} = {\cal L}_1 \dot{u}
    +{\cal L}_2 {\cal L}_3 u
    +{\cal L}_2 {\cal L}_4 \left(
     {\cal L}_2^{-1} (\dot{u} - {\cal L}_1 {u})
    \right)
\end{equation}
%
where (\ref{eq:linearPDE2}a) is differentiated with respect to time and (\ref{eq:linearPDE2}b) is used in order to write the PDEs as a function of $u(x,t)$ alone.  Thus knowledge of the field $u(x,t)$ alone is capable of constructing the solution fields $u(x,t)$ and $v(x,t)$.  For this second-order (in time) PDE, both an initial condition $u(x,0)$ and an initial {\em velocity} require specification 
$\dot{u}(x,0)$ in order to uniquely determine the solution.  As with the previous arguments, a time trajectory embedding of $2N$ measurements can be used to uniquely determine the solution.


